Kernel-estimated Nonparametric Overlap-Based Syncytial Clustering

Commonly-used clustering algorithms usually find ellipsoidal, spherical or other regular-structured clusters, but are more challenged when the underlying groups lack formal structure or definition. Syncytial clustering is the name that we introduce for methods that merge groups obtained from standard clustering algorithms in order to reveal complex group structure in the data. Here, we develop a distribution-free fully-automated syncytial clustering algorithm that can be used with $k$-means and other algorithms. Our approach estimates the cumulative distribution function of the normed residuals from an appropriately fit $k$-groups model and calculates the estimated nonparametric overlap between each pair of clusters. Groups with high pairwise overlap are merged as long as the estimated generalized overlap decreases. Our methodology is always a top performer in identifying groups with regular and irregular structures in several datasets and can be applied to datasets with scatter or incomplete records. The approach is also used to identify the distinct kinds of gamma ray bursts in the Burst and Transient Source Experiment 4Br catalog and the distinct kinds of activation in a functional Magnetic Resonance Imaging study.

==> simulation.tex <==
\section{Performance Evaluations}
\label{sec:eval}
We first illustrate the performance of KNOB-SynC on a two-dimensional
\texttt{Aggregation} dataset of 
\citet{gionis07} and then follow up with more detailed performance
evaluations with a large number of datasets in the literature. These
datasets ranged from two to many dimensions. We compared our methods
with a bunch of clustering methods. Among these were the syncytial
clustering techniques of K-mH~\citep{petersonetal17} using
author-supplied {\sf R} code,
MMC~\citep{baudryetal10} as implemented in  
the {\sc R} package {\sc MixModCombi}, DEMP~\citep{hennig10} 
using the {\sc R} package {\sc fpc} and DEMP+~\citep{melnykov16}. In
addition, we also evaluated performance using
EAC~\citep{fredandjain05}, the generalized single linkage with nearest
neighbor (GSL-NN) density estimate of ~\citep{stuetzleandnugent10}
using their supplied code from the 
supplementary materials of the journal website.
We also used two common connectivity-based techniques
of spectral and kernel $k$-means clustering. Both methods need the
number of groups to proceed: for spectral clustering we decided on the
number of groups to be the one with 
the highest gap in successive eigenvalues of the similarity
matrix~\citep{vonluxburg07}. For kernel $k$-means, we chose $K$ to be
known at the true value: we recognize that our evaluation of kernel
$k$-means provides this method with an unfair advantage, however, we
proceed in this fashion in order to understand the best case scenario
of this competing method. For all datasets and cases we evaluated
performance in terms of the adjusted Rand index ${\mR}$
\citep{hubertandarabie85} between the true partition and the  
estimated final partitioning using each method. The index $\mR$ takes
values in $(-\infty, 1]$ with values closer to 1 indicating greater
similarity between partitionings and good 
clustering performance and conversely values substantially below 1 indicating
poorer clustering performance.  

%Implementation of FJ was done using the built-in \texttt{R} functions \texttt{hclust()} and \texttt{kmeans()}. The number of groups were determined based on \citep{fredandjain05}. Baudry merge done using the \texttt{R} package {\it RmixmodCombi}, ~\citep{RmixmodCombi}. \citep{baudryetal10} does not provide a conventional formal statistical inferential method for choosing between different numbers of clusters but suggested a method based on the ''elbow rule''. To perform GSL-NN, we use the \texttt{R} code provided in the supplemental material of \citep{stuetzleandnugent10}. DEMP was done using the \texttt{R} package {\it fpc}, ~\citep{fpc}, and DEMP+ was done computed using the package \texttt{mclust}. Figure \ref{fig:realdata} display all the 2-dimensional datasets used as experimental. The data set \texttt{aggregation} from ~\citep{gionis07}, consist in a two dimensional seven groups. \texttt{Compound}, ~\citep{zahn71}, consist in a 6 group dataset with different structures. From ~\citep{chang08}, \texttt{pathbased} and \texttt{spiral}, \texttt{D31} and \texttt{R15} ~\citep{veenman02}, \texttt{Jain} ~\citep{jain05}, \texttt{FLAME} ~\citep{fu07}. All the mentioned datasets are shape datasets that require clustering connectivity rather than partition such as $k$-means. Other datasets consist the bullseye, and bananas-clump from ~\citep{stuetzleandnugent10}.
%some datasets. We used 16 2-dimensional datasets and 9 datasets with dimension larger than 2. For all the datasets the initial partition was obtained using $k$-means $k = 1,\ldots, K_{\max}= \max\{\sqrt{n},50\}$. From this range of $k$ cluster we determined the optimal partition using the jump method, call it $K_0 = \hat{K}$. We applied KNOB-SynC starting from $K_0$ and following the described methodology. 
\subsection{Illustrative Example: the \texttt{Aggregation} dataset}
\begin{figure*}
  \centering
%  \subfloat[]{\includegraphics[width=0.35\textwidth]{figures/Example-Step-1.pdf} }
%  \caption{True dataset before applying $k$-means.}
\mbox{
  \subfloat[$k$-means phase end: $\hat K=14$]{\includegraphics[width=0.33\textwidth]{figures/Example-Step-1-K-14}
    \label{fig:kmeans.step.1}}
  \subfloat[First merging phase end: $\hat K=8$]{\includegraphics[width=0.33\textwidth]{figures/Example-Step-2-K-8}\label{fig:kmeans.step.3}}
  \subfloat[Final solution: $\hat K=7$]{\includegraphics[width=0.33\textwidth]{figures/Example-Step-3-K-7}\label{fig:kmeans.step.5}}}
\mbox{
  \subfloat[$k$-means end: $\genhatomega=0.0013$]{\includegraphics[width=0.33\textwidth]{figures/Example-Step-Overlap-Matrix-K-14}\label{fig:overlap.step.2}}
  \subfloat[Merging phase I: $\genhatomega=0.0008$]{\includegraphics[width=0.33\textwidth]{figures/Example-Step-Overlap-Matrix-K-8}\label{fig:kmeans.step.4}}
\subfloat[\!Final solution: $\!\!\genhatomega\!\!=\!\!10^{-6};\mR=0.98$]{\includegraphics[width=0.33\textwidth]{figures/Example-Step-Overlap-Matrix-K-7}\label{fig:kmeans.step.6}}}
\mbox{\subfloat[]{\includegraphics[width = \textwidth]{figures/Example-Aggregation-Competitors}\label{fig:aggregation}}}
\caption{(a)-(f) Illustrating of the KNOB-SynC algorithm on the {\tt
    Aggregation} dataset, and (g) groups obtained using competing
  algorithms. In all cases, 
character denotes true class membership which color indicates
estimated class membership.}
\label{fig:merging.step.1}
\end{figure*}
The two-dimensional \texttt{Aggregation} dataset \citep{gionis07} has
$n=788$ observations from $C=7$ groups of different
characteristics. Figure~\ref{fig:merging.step.1} 
displays the results of the different phases and iterations of
KNOB-SynC and performance with competing methods. The stages of
KNOB-SynC are displayed for $\kappa=1$ which
is also the one that had the lowest terminating $\hat{\ddot\omega}$
(from among $\kappa = 1,2,3,\infty$).  In this and other similar
figures in this paper, plotting color and character  represent the
estimated and true group identifications, respectively. The $k$-means
phase of our algorithm identifies 14 clusters with partitioning as in
Figure~\ref{fig:kmeans.step.1} and the initial overlap matrix
$\hat\Omega$ of Figure~\ref{fig:overlap.step.2}. The first merging phase yields
the partitioning  in Figure~\ref{fig:kmeans.step.3} with the updated
$\hat\Omega$ of Figure~\ref{fig:kmeans.step.4}. The next merging phase only
merges one pair of groups and is terminal, resulting in the final
partitioning of the dataset as in Figure~\ref{fig:kmeans.step.5}. The
overlap matrix (Figure~\ref{fig:kmeans.step.6}) indicates
well-separated clusters. Only two observations are mislabeled,
yielding a $\mR$ of 0.98 between the true and estimated
classification.

The competing methods (Figure~\ref{fig:aggregation}) all perform
marginally to substantially worse. K-mH is the second best performer
($\mR=0.95$), finding $\hat C=9$ groups, but breaking the top right 
cluster into two and also grouping a few other stray
observations. Both DEMP and DEMP+ yield the same result ($\mR=0.91,
\hat C = 6$), but MMC has trouble with the largest group, splitting it
into two, with $\mR=0.8$ and $\hat C = 8$. EAC breaks the top
central and large
groups on the right into many clusters, resulting in $\hat C = 14$ but
$\mR = 0.9$. Thus, in spite of the large number of groups, EAC is able
to capture quite a bit of the complicated
structure  of this dataset. GSL-NN can not distinguish between the groups on the
right but finds many small groups elsewhere, ending up with $\hat
C =12 $ and $\mR = 0.81$. Spectral clustering performs worse,
finding $\hat C = 12$ groups with $\mR = 0.59$. Despite being supplied
the true $C=7$, kernel $k$-means with $\mR=0.18$ is the worst
performer in this example.

\begin{comment}
\begin{figure*}[h!]
  \centering
  \includegraphics[width = \textwidth]{figures/Aggregation-2D}
  \caption{Clustering algorithm on the 8 different input clustering on the datasets \texttt{Aggregation}.}\label{fig:aggregation}
\end{figure*}

\begin{comment}
We first determine the optimal number of
homogeneous group in the datasets based on $k$-means and the jump
methodology and $y = p/2$, although the choice of $y$ seems arbitrary,
see \citet{sugarandjames03} for a more detail discussion about
it. Jump method determined that the optimal number of groups to be
$K_0 = 14$,. In Figure \ref{fig:kmeans.step.2} we obtain
homogeneous. We treat this $K_0 = 14$ as our initial clusters to be
merge. Using kernel estimator proposed in Equation ~\eqref{}. In
Figure \ref{fig:overlap.step.3} display the overlap matrix
$\hat{\Omega}$ for this $K_0 = 14$ initial clusters. The generalized
overlap  $\hat{\Omega}$ is $\genomega = 0.005$. The clusters with the
highest interaction will be merge. In the overlap matrix it can be
seen that cluster 1 is likely to be merge with cluster 3 and follow
with cluster 14. Cluster 2 will be merge with cluster 4 and 11. For
the rear 
\end{comment}

\subsection{Additional 2D Experiments}
\subsubsection{Experimental framework}
Figure~\ref{fig:2ddata} displays the 12 additional 2D
datasets used to evaluate performance of KNOB-SynC and its
competitors. Many of these datasets have been used by other authors to
\begin{figure*}[h]
  \centering
  \includegraphics[width = \textwidth]{figures/Datasets-display-3x4-Shapes}
  \caption{Shape datasets used in the two-dimensional performance
    evaluations.}
  \label{fig:2ddata}
\end{figure*}
demonstrate and evaluate performance of their methods. The groups in
these datasets have structure ranging from the regular (see {\em
  e.g.}, the 7-spherically-dispersed Gaussian clusters dataset that is 
modeled on a similar example in \citep{maitra09}) to widely-varying
complexity. The {\tt Banana Arcs} dataset has $n=4515$ observations
clumped in four banana-shaped structures 
arced around each other. The {\tt Banana-clump} and {\tt Bullseye}
datasets were used in \citet{stuetzleandnugent10} and
\citet{petersonetal17} -- the former has 200 observations with one
spherical group and another arced around it on the left like a
banana, while the latter has 400 observations grouped, as its
name implies, as a bullseye.  The more complex-structured {\tt
  Bullseye-Cigarette} dataset \citep{petersonetal17} has three 
concentric ringed groups, two elongated groups above two spherical
groups on the left, and another group that is actually a superset of
two overlapping spherical groups ($n=3025$ and $C=8$). The
{\tt Compound} dataset~\citep{zahn71} is very complex-structured
with $n=399$ observations in $C=6$ groups that are not just
varied in shape, but a group that sits atop another on the right. The
{\tt Jain} dataset~\citep{jainandlaw05} has 373 observations in two
arc-shaped clusters, one of which is dense and the other very
sparsely-populated. The {\tt Pathbased} dataset~\citep{veenman02} has
300 observations in three groups, two of which are regular-shaped and
surrounded by a widely arcing third group.  The {\tt   Spiral}
dataset~\citep{veenman02} has 312 observations in three spiral groups 
that very difficult for standard clustering algorithms to recover. The
{\tt SSS} dataset has 5015 observations in 
three S-shaped groups of varying density and orientations while the
{\tt XXXX} dataset has $n=415$ observations
distributed in four cross-shaped structures in the dataset.
\subsubsection{Results}
Figure~\ref{fig:AR.2d} and Table~\ref{tab:AR.2d} summarizes the
results of all the methods in the 2-dimensional experimental
datasets.  Detailed displays of different methods 
 (with the exception of kernel $k$-means, which we skip for
\begin{figure}[h!]
  \centering
  \includegraphics[width = \textwidth]{figures/AR}
  \caption{Performance, in terms of the Adjusted Rand Index, of all
    methods on 2D datasets.}
  \label{fig:AR.2d}
\end{figure}
\begin{table*}[h!]
  \centering
  \caption{Performance, in terms of ${\cal R}$ and estimated $\hat C$,
    on 2D datasets, of competing methods: KNOB-SynC (denoted as KNS in the
    table), K-mH, DEMP (DM), DEMP+ (DM+), MMC, EAC, GSL-NN
    (GSN), spectral clustering (SpC) and kernel-$k$-means
    (k-$k$m). For k-$k$m, $\hat C$ was set at the true $C$ and not
    estimated. 
    For each method, the absolute deviation of $\mR$
    for that method from the highest $\mR$ for each dataset was
    obtained: the average and SD of these absolute deviations are also
    reported for each method in the last row.}
  \label{tab:AR.2d}
  \begin{tabular}{lrrrrrrrrrr}
    \hline\hline
    Dataset & & KNS & K-mH& DM & DM+ & MMC & EAC & GSN  & SpC & k-$k$m \\
    $(n,p,K)$ & &  & &  & &  &  &  & &  \\
    \hline\hline
    7-Spherical & ${\cal R}$ & 0.98 & 0.89 & 1.00 & 1.00 & 0.63 & 0.82 & 0.69 & 0.86 & 0.82\\
     $(500,2,7)$ & $\hat{C}$ & 7 & 10 & 7 & 7 & 5 & 9 & 10 & 7 & \\
    \hline
    Aggregation&${\cal R}$ & 0.98 & 0.93 & 0.91 & 0.91 & 0.83 & 0.94 & 0.81 & 0.84 & 0.18\\
    $(788,2,7)$  &$\hat{C}$ & 7 & 9 & 6 & 6 & 5 & 12 & 11 & 7 & \\
    \hline
    Banana-arcs&${\cal R}$ & 0.91 & 1.00 & 0.5 & 0.54 & 0.13 & 1.00 & 1.00 & 1.00 & 0.16\\
     $(4515,2,4)$       &$\hat{C}$ & 5 & 1 & 15 & 10 & 39 & 6 & 6 & 4 & \\
    \hline
    Banana-clump&${\cal R}$ & 0.99 & 1.00 & 0.77 & 1.00 & 0.62 & 1.00 & 0.99 & 1.00 & 0.98\\
     $(200,2,2)$       &$\hat{C}$ & 3 & 2 & 3 & 2 & 5 & 2 & 3 & 3 & \\
    \hline
%    Bananas-sphere&${\cal R}$ & 0.50 & 0.69 & 0.29 & 0.45 & 0.10 & 1.00 & 1.00 & 1.00 & 0.63\\
%     $(3015,2,3)$       &$\hat{K}$ & 3 & 3 & 14 & 11 & 32 & 4 & 3 & 3 & 3\\
%    \hline
    Bullseye&${\cal R}$ & 1.00 & 0.92 & 0.21 & 0.31 & 0.20 & 0.51 & 0.99 & 1.00 & 0.22\\
     $(400,2,2)$       &$\hat{C}$ & 2 & 2 & 7 & 5 & 10 & 5 & 3 & 2 & \\
    \hline
    Bullseye-cig&${\cal R}$ & 0.99 & 0.62 & 0.64 & 0.37 & 1.00 & 1.00 & 0.38 & 0.82 &0.38 \\
    $(3025,2,8)$       &$\hat{C}$ & 7 & 6 & 7 & 7 & 5 & 9 & 15 & 7 & \\
    \hline
    Compound&${\cal R}$ & 0.93 & 0.5 & 0.74 & 0.74 & 0.59 & 0.85 & 0.77 & 0.39 & 0.26 \\
     $(399,2,6)$       &$\hat{C}$ & 19 & 12 & 3 & 3 & 3 & 8 & 14 & 16 & \\
    \hline
%    D31&${\cal R}$ & 0.95 & 0.87 & 0.83 & 0.79 & 0.70 & 0.21 & 0.51 & 0.74 & 0.51\\
%     $(3100,2,31)$       &$\hat{K}$ & 7 & 6 & 7 & 7 & 5 & 9 & 15 & 7 & 31\\
%    \hline
%    Flame&${\cal R}$ & 0.89 & 0.44 & 0.00 & 0.00 & 0.00 & 0.48 & 0.91 & 0.21 & 0.5\\ 
%    $(240,2,2)$        &$\hat{K}$ & 5 & 12 & 1 & 1 & 1 & 5 & 12 & 2 & 2\\
%    \hline
    Jain&${\cal R}$ & 0.88 & 0.95 & 0.37 & 0.37 & 0.12 & 1.00 & 0.94 & 1.00 & 0.01\\
     $(373,2,2)$       &$\hat{C}$ & 16 & 3 & 6 & 6 & 11 & 2 & 4 & 2 & \\
    \hline
    Pathbased&${\cal R}$ & 0.55 & 0.42 & 0.41 & 0.41 & 0.41 & 0.45 & 0.59 & 0.77 & 0.23 \\
    $(300,2,3)$        &$\hat{C}$ & 21 & 2 & 2 & 2 & 3 & 15 & 6 & 3 & \\
    \hline
%    R15&${\cal R}$ & 0.99 & 0.07 & 0.99 & 0.99 & 0.92 & 0.90 & 0.79 & 0.75 & 0.82 \\
%    $(600,2,15)$        &$\hat{K}$ & 15 & 4 & 15 & 15 & 14 & 19 & 19 & 17 & 16\\
%    \hline
    SCX-Bananas&${\cal R}$ & 0.95 & 1 & 0.81 & 0.79 & 0.19 & 1.00 & 1.00 & 0.57 & 0.41\\
     $(3420,2,8)$       &$\hat{C}$ & 8 & 8 & 7 & 9 & 39 & 8 & 8 & 4 & \\
    \hline
    Spiral&${\cal R}$ & 0.86 & 0.01 & 0.00 & 0.00 & 0.00 & 0.18 & 1.00 & 1.00 & 0 \\
      $(312,2,3)$      &$\hat{C}$ & 3 & 2 & 1 & 1 & 1 & 9 & 3 & 3 & \\
    \hline
    SSS &${\cal R}$& 1.00 & 0.77 & 0.77 & 0.84 & 0.63 & 1.00 & 1.00 & 0.2 & 0.23\\
    $(5015,2,3)$        &$\hat{C}$ & 3 & 5 & 5 & 4 & 27 & 4 & 3 & 19 & \\
    \hline
    XXXX &${\cal R}$& 0.95 & 0.65 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.30 & 0.97\\
     $(415,2,4)$       &$\hat{C}$ & 10 & 6 & 4 & 4 & 4 & 4 & 4 & 20 & \\
    \hline\hline
%    $\bar{\cal D}$ & & 0.105 &  0.218 &  0.348 & 0.335& 0.488& 0.159& 0.11& 0.245 & 0.591 \\
%    ${\cal D}_\sigma$ & & 0.207&0.279&0.310&0.322&0.353 & 0.273 & 0.18                                                      & 0.293& 0.331    \\
        $\bar{\cal D}$ & & 0.052 &  0.118 &  0.348 & 0.316& 0.552 & 0.159& 0.062 & 0.29 & 0.591 \\
    ${\cal D}_\sigma$ & & 0.055 &0.280 & 0.310 &0.311 &0.331 & 0.273 & 0.097 & 0.326 & 0.331 \\
%    Median ${\cal D}$ & & 0.05&0.05 &0.23&0.21&0.38 &0.01 & 0.01 & 0.14 & 0.67\\
%    IQR ${\cal D}$ & &   0.09 &0.26 &0.38&0.43&0.51&0.18 &0.09 &0.54 & 0.33 \\

\hline  \hline  
  \end{tabular}
\end{table*}
 compactness of the figure, and also because of its need for given
 $K$) on individual datasets are in Appendix~\ref{appendix-2D}. The
 summaries indicate across-the-board good performance of KNOB-SynC, in
 terms of $\mR$, with it being close to the top in almost all
 cases. In its worst case here, KNOB-SynC gets a $\mR=0.55$ on the
 {\tt Pathbased} dataset because it terminates
 early~(Figure~\ref{fig:pathbased}), but here also 
 it is the third-best performer, behind spectral clustering
 ($\mR=0.77$) and EAC ($\mR=0.59$). 
 The competing syncytial clustering methods do well in some
 cases, but not in others where the other comparison methods
 perform better. Among the syncytial clustering methods, K-mH perform
 better than  DEMP, DEMP+  and MMC whose  performance
 can be poor in some cases ({\em e.g.}, on the
{\tt Bullseye} and {\tt Jain} and {\tt Spiral} datasets of
\ref{fig:Bullseye}, \ref{fig:Jain} and \ref{fig:spiral},
respectively). It is on these datasets that the other methods 
(EAC, GSL-NN, Spectral clustering) do better. The performance of
kernel-$k$-means is varied, even with known true number of groups,
being very good sometimes ({\em
  e.g.}, in the {\tt Bananas-clump} dataset of
Figure~\ref{fig:Bananas}) but very poor in cases ({\em e.g.}, as seen
before in the {\tt   Aggregation} dataset) where every 
other method does well. We quantify performance of each method against
its competitors in terms of its average deviation from the best
performer. Specifically, for each dataset, we compute the difference
in $\mR$ of a method from that of the best performer for that
dataset. We call these deviations. The average deviation ($\bar
{\mathcal D}$) of a method over all datasets is an overall indicator
of its performance.Table~\ref{tab:AR.2d} provides
$\bar{\mathcal D}$ and the standard deviation ($\mathcal D_\sigma$) of
the differences.  On the average,  KNOB-SynC is the
best performer (also having the lowest $\mathcal D_\sigma$) followed
by GSL-NN, K-mH and EAC. We surmise that KNOB-SynC does 
well across the different kinds of datasets because of its ability
by construction to merge many or few components at a time, with the
exact choice and termination completely data-driven and objective and
determined by the distinctiveness of the resulting partitioning
as measured by $\genhatomega$. 

 \begin{comment}


 Figure \ref{fig:realdata} display all the 2-dimensional datasets used
 as experimental. The data set \texttt{aggregation} from
 ~\citep{gionis07}, consist in a two dimensional seven
 groups. \texttt{Compound}, ~\citep{zahn71}, consist in a 6 group
 dataset with different structures. From ~\citep{chang08},
 \texttt{pathbased} and \texttt{spiral}, \texttt{D31} and \texttt{R15}
 ~\citep{veenman02}, \texttt{Jain} ~\citep{jain05}, \texttt{FLAME}
 ~\citep{fu07}. All the mentioned datasets are shape datasets that
 require clustering connectivity rather than partition such as
 $k$-means. Other datasets consist the bullseye, and bananas-clump
 from ~\citep{stuetzleandnugent10}. The {\tt SCX}
 dataset~\citep{petersonetal17} has $n=3,420$ observations in $K=7$
 groups of varying shapes, sizes and structure, with four-small
 X-shaped groups on the left quadrant, three C-shaped
 groups rotated at different angles on the right and one large
 S-shaped group running from top to bottom on the left.


%We studied the performance of each methodology, specially of KNOB-SynC, with different ''bananas'' structures. This 2-dimensional data consist of two separated groups each resembling a banana each banana group contains 750 observation. The banana-shaped groups are surrounded by a third group in the shape of a full ring composed of 1500 observations. In addition 15 randomly scattered points are added to this dataset for a total of 3015 observations. Figure \ref{fig:banana.Sphere} display the results for each of the methodologies, next of the name of the methodology is the reported Adjusted Rand Index ${\cal R}$. Similarly display of results is for the \texttt{Bananas-Arcs}. For this datasets we have for separate groups, two groups resembling a banana in the middle. The other two groups are a outside curve arcs.  For these datasets our methodology perform excellent obtaining  ${\cal R}= 1$. for this case, our biggest competitors are FJ, and GSL-NN. The lowest performance for each data was obtained for MMC.


 
\begin{figure}[h!]
  \centering
  \includegraphics[width = \textwidth]{figures/G7-2D}
  \caption{Clustering algorithm on the 8 different input clustering on the datasets \texttt{G7}.}
  \label{fig:g7}
\end{figure}

\begin{figure*}
  \centering
  \includegraphics[width = \textwidth]{figures/Banana-Arcs-2D}
  \caption{Clustering algorithm on the 8 different input clustering on the datasets \texttt{banana-arcs}.}
  \label{fig:banana.arcs}
\end{figure*}

\begin{figure*}
  \centering
  \includegraphics[width = \textwidth]{figures/Bananas-Sphere-2D}
  \caption{Clustering algorithm on the 8 different input clustering on the datasets \texttt{bananas-sphere}.}
  \label{fig:banana.Sphere}
\end{figure*}

\begin{figure*}
  \centering
  \includegraphics[width = \textwidth]{figures/Bananas-clump-2D}
  \caption{Clustering algorithm on the 8 different input clustering on the datasets \texttt{Bananas-clump}.}
  \label{fig:Bananas}
\end{figure*}
\begin{figure*}
  \centering
  \includegraphics[width = \textwidth]{figures/Bullseye-2D}
  \caption{Clustering algorithm on the 8 different input clustering on the datasets \texttt{bullseye}.}
  \label{fig:Bullseye}
\end{figure*}

\begin{figure*}
  \centering
  \includegraphics[width = \textwidth]{figures/Bullseye-Cigarette-2D}
  \caption{Clustering algorithm on the 8 different input clustering on the datasets \texttt{Bullseye-cigarette}.}
  \label{fig:Bullseye-Cigarette}
\end{figure*}


\begin{figure}
  \centering
  \includegraphics[width = \textwidth]{figures/Compound-2D}
  \caption{Clustering algorithm on the 8 different input clustering on the datasets \texttt{compound}.}
  \label{fig:compound}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width = \textwidth]{figures/D31-2D}
  \caption{Mixture of Gaussian data set \texttt{D31}.}
  \label{fig:d31}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width = \textwidth]{figures/Flame-2D}
  \caption{Clustering algorithm on the 8 different input clustering on the datasets \texttt{flame}.}
  \label{fig:flame}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width = \textwidth]{figures/Jain-2D}
  \caption{Clustering algorithm on the 8 different input clustering on the datasets \texttt{Jain}.}
  \label{fig:Jain}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width = \textwidth]{figures/Pathbased-2D}
  \caption{Clustering algorithm on the 8 different input clustering on the datasets \texttt{pathbased}.}
  \label{fig:pathbased}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width = \textwidth]{figures/R15-2D}
  \caption{Mixture of Gaussian data set \texttt{R15}.}
  \label{fig:r15}
\end{figure}

\begin{figure*}
  \centering
  \includegraphics[width = \textwidth]{figures/SCX-Bananas-2D}
  \caption{Clustering algorithm on the 8 different input clustering on the datasets \texttt{SCX-Bananas}.}
  \label{fig:SCX}
\end{figure*}

\begin{figure}
  \centering
  \includegraphics[width = \textwidth]{figures/Spiral-2D}
  \caption{Clustering algorithm on the 8 different input clustering on the datasets \texttt{Spiral}.}
  \label{fig:spiral}
\end{figure}

\begin{figure*}
  \centering
  \includegraphics[width = \textwidth]{figures/SSS-2D}
  \caption{Clustering algorithm on the 8 different input clustering on the datasets \texttt{SSS}.}
  \label{fig:SSS}
\end{figure*}

\begin{figure*}
  \centering
  \includegraphics[width = \textwidth]{figures/XXXX-2D}
  \caption{Clustering algorithm on the 8 different input clustering on the datasets \texttt{XXXX}.}
  \label{fig:XXXX}
\end{figure*}

The next examples are are taken from \citet{stuetzleandnugent10}. The
Banana-clump dataset consist of a Gaussian cloud and a banana-shaped
group with a total of 200 observations. The Bullseye Dataset consists
of a Gaussian cloud surrounded by a spherical cluster with a total of
400 observations, their data and code is available at the journal
website as part of the supplemental material. The first dataset is the
bullseye data. Figure \ref{fig:Bullseye} our algorithm seems to
recover both groups the ${\cal R} = 0.92$ for the final merging
step. Figure \ref{fig:Bananas} contained the results for the proposed
merging algorithm. At the first merging step the algorithm Adjusted
Rand index ${\cal R} = 0.59$, and the final merging step the adjusted
Rand index ${\cal R} = 1$. The examples in this section were created
to showcase datasets using a variety of cluster shapes with different
cluster sizes. The SCX dataset contains three separated C-shaped
groups rotated at different angles, a large S-shaped group and four
small x-shaped groups. In addition 20 randomly scattered points are
added to the dataset for a total of 3420 observations. The
Cigarette-Bullseye dataset consists of three concentric rings, two
long clusters above two small clusters and one cluster that is formed
using two overlapping Gaussian groups. The data set
\texttt{aggregation} from ~\citep{gionis07}, consist in a two
dimensional. The second is \texttt{compound} ~\citep{zahn71},
\texttt{pathbased} and \texttt{spiral} ~\citep{chang08}, \texttt{D31}
and \texttt{R15} ~\citep{veenman02}, \texttt{Jain} ~\citep{jain05},
\texttt{FLAME} ~\citep{fu07}. 
\end{comment}

\subsection{Higher-Dimensional Datasets}
%Having evaluated performance on two-dimensional examples, we now
%investigate KNOB-SynC in relation to other methods on some higher-dimensional datasets.
We also studied the performance of KNOB-SynC and its competitors in
higher-dimensional datasets. These datasets are modest to higher-dimensional
and range in size from over 173 to 10993.
For the higher-dimensional datasets (Acute Lymphoblastic Leukemia and Zipcode
digits), we found that all methods other than GSL-NN perform
better when used on the first few ($m$) kernel principal components
(KPCs) rather than on the raw data. For these methods and these
datasets therefore, we used the 
first $m$ KPCs of each dataset with $m$ chosen as the first time after which 
increases in the eigenvalues corresponding to the successive KPCs are
below 0.5\%. GSL-NN was evaluated on the original datasets. 
We describe the datasets and
performance in the next sections and summarize performance on all the
datasets in Section~\ref{sec:HD}.
\begin{comment}
For the higher-dimensional datasets such
as ALL and Zip digits, we found
that all methods other than GSL-NN perform better when used on the
first few ($m$) kernel principal components (KPCs) rather than the raw
data. For these methods and these datasets therefore, we used the
first $m$ KPCs of each 
dataset with $m$ chosen as the first time after which 
increases in the eigenvalues corresponding to the successive KPCs are
below 0.5\%. GSL-NN was evaluated on the original datasets here. For
the moderately-sized Image and Pen Digits datasets, we used the first
PCs that explained at least 99.97\% of the dataset. For the remaining 
modest-dimensional datasets, we used the raw observations for all the
methods. 
\begin{comment}

For the
image and the Handwritten Digits datasets, we 
We used the
KPCs for all but the Handwritten Digits dataset where it was not
possible to get the KPCs extracted in a reasonable time: we refer to
Section~\ref{sec:pen.digits} for more details.
\end{comment}

\subsubsection{Simplex-7 Gaussian Clusters}
This dataset, from \citet{stuetzleandnugent10}, is of Gaussian
realizations of size 50, 60, 70, 80, 90, 100 and 110 each
from seven clusters with means set at the vertices of the
seven-dimensional unit simplex and homogeneous spherical dispersions
with common standard deviation of 0.25 in each dimension. Like the
{\tt 7-Spherical} dataset, it is an example of a case where standard
methods such as $k$-means or Gaussian-mixture-model-based clustering
should be  adequate. Therefore it is a test of whether our algorithm
and its competitors are able to refrain from
identifying spurious complexity. All methods identify seven groups and
have good clustering performance. In particular, the syncytial methods
have very good performance ($\mR=0.97$) and only marginally better
than the others (then $0.92\leq\mR\leq0.94$).

\subsubsection{E. coli Protein Localization}
The {\em E. coli} dataset, publicly  available from the University of
California Irvine's 
Machine Learning Repository (UCIMLR)~\citep{newmanetal98}. concerns identification of
protein localization sites for the {\em E. coli}  bacteria, an
important early step  for finding
remedies~\citep{nakaiandkinehasa91}. There are eight protein
localization sites: cytoplasm, inner membrane without signal sequence,  periplasm, or inner membrane with an uncleavable signal sequence, 
outer membrane, outer membrane lipoprotein, 
inner membrane lipoprotein or  inner membrane with a
cleavable signal sequence. Identifying these sites is an important
early step for finding remedies~\citep{nakaiandkinehasa91}. 
Each protein sequence has a number of numerical attributes -- see
\citet{hortonandnakai96} for a listing and
their detailed description. Two attributes are
binary, but 326 of the 336 sequences have common values for these
attributes. We restrict our investigation to these sequences and drop
these two attributes from our list of variables. These 326 sequences have
no representation from the inner membrane or outer membrane
lipoproteins. Additionally, we also drop two sequences because they
are the lone representatives from the inner membrane with cleavable
sequence site~\citep{maitra02}. 
\begin{table}[ht]
\centering
\caption{Confusion matrix of the KNOB-SynC grouping against the true for the {\em E. coli} dataset.}
\label{tab:knob.sync.Ecoli-unscaled-5-kappa-5}
\begin{tabular}{lrrrrrrrrr}
  \hline
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 \\
  \hline
cytoplasm &   138 & 0 &  0 & 4 &   0 &   0 &   0 &   0 &    1 \\
  inner membrane, no signal sequence &  7 & 62  & 0 &  0 &   0 &   3 &   3 &   1 &   0 \\
  inner membrane, uncleavable signal sequence & 1 & 32 &  0 & 0 &   0 &   0 &   0 &   1 &   0  \\
  outer membrane &   0 &   0 & 17 &  2 &   0 &   0 &   0 &   0 &     0 \\
  periplasm &   3 &   1 &  2 & 38 &   8 &   0 &   0 &   0 &     0 \\
   \hline
\end{tabular}
\end{table}
Therefore we have $n=324$ observations from $C=5$ true classes. For
this example KNOB-SynC identifies $\hat C = 9$
groups. Table~\ref{tab:knob.sync.Ecoli-unscaled-5-kappa-5} presents
the confusion matrix containing the number of cases a protein from a
localization site was assigned to KNOB-SynC group. 
Ignoring stray
assignments, the sites are fairly well-defined in the first four
groups, with $\mR=0.72$. Uncleavable signal sequences 
from the inner membrane site are difficult to distinguish from those
that are also from there but have no signal
sequence. Sequences from the other sites are better-clarified. 
Among the alternative methods, EAC does slightly better ($\mR=0.77)$
but identifies 10 groups. The remaining methods all do slightly  to
substantially worse. DEMP, DEMP+ and K-mH each identify four groups
but with $\mR\in [0.63,0.78]$. K-mH finds only two groups ($\mR=0.41$)
while the rest find more groups but disagree more strongly with the
true localization. Thus EAC and KNOB-SynC are the top two
performers for this dataset.
  

\subsubsection{Wine Recognition} \label{sec:app.wine}
The wine recognition dataset~\citep{forinaetal88,aeberhardetal92} also
obtainable from the UCIMLR
contains $p=13$ measurements on $n=178$  wine samples that are
obtained from 
its chemical analysis. There are 59, 71 and 48 wines of the Barolo,
Grignolino  and Barbera cultivars, respectively, so $C=3$. KNOB-SynC
is a middling performer for this dataset, finding  $\hat C=24$ groups
with a clustering performance of $\mR=0.55$. All 48 members of the
largest identified group are from the Barola cultivar while all 42
members of the second group are from the Grignolino cultivar. The
third group has two Grignolino wines and 35 wines from the Barbera
cultivar. Thus, there is fairly good definition among these
groups. However, there are a large number of very small groups also
identified which explains the reduced clustering performance. Among
competitors, only MMC ($\mR = 0.67; \hat C = 5$), K-mH ($\mR =
0.62,\hat C = 6$) and EAC ($\mR = 0.60;\hat C = 9$) do better and
the others do marginally to moderately worse.
\begin{comment}
27 variables:
Alcohol, Sugar-free extract, Fixed acidity, Tartaric acid, Malic acid
of wine belonging to the same region in Italy but using different cultivars. This data set is a well known use in classification problem to determine the performance of a new classification technique. The classes in this data set are the three types of wine, wine 1 contain 59 observations, Wine 2 71 and Wine 3 48. Kernel principal components analysis was performed before applying $k$-means the initial number of groups $K_0=49$. KNOB-SynC determine 24 different type of wines adjusted Rand Index ${\cal R}  = 0.556$ and $\ddot{\omega} = 0.00031$. Table \ref{tab:knob.sync.wine} display a 

\begin{table}[ht]
  \centering
\caption{Confusion matrix for Wines dataset, KNOB-SynC determine 24 cluster solution.}  \label{tab:knob.sync.wine}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrr}
  \hline
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 \\ 
  \hline
  Wine 1 &  48 &   0 &   0 &   6 &   0 &   2 &   3 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 \\ 
  Wine 2 &   0 &  42 &   2 &   0 &   1 &   0 &   0 &   1 &   3 &   2 &   3 &   3 &   2 &   1 &   1 &   2 &   1 &   2 &   1 &   1 &   2 &   1 &   0 &   0 \\ 
  Wine 3 &   0 &   0 &  35 &   0 &   8 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   3 &   2 \\ 
   \hline
\end{tabular}
\end{table}
\end{comment}

\subsubsection{Olive Oils}
\label{sec:olives}
The olive oils dataset~\citep{forinaandtiscornia82,forinaetal83} has
measurements on 8 chemical components for 572 samples of olive oil
taken from 9 different areas in Italy which are from three regions:
Sardinia and Northern and Southern Italy. This is an interesting
dataset with sub-classes (areas) inside classes (regions). Indeed,
\citet{petersonetal17} were able to identify sub-groups within the
regions with one misclassification
but not the areas ($\mR=0.67, \hat C=11$; we however found
$\mR=0.56, \hat C=8$  using the authors' supplied code): they surmised
that it may be more possible to identify characteristics of olive oils
based on regions based on physical geography rather than
areas based on political geography. We therefore analyze
performance on this dataset in terms of how both regions and
areas are recovered. KNOB-SynC identifies four 
regions with oils from the Sardinian and Northern regions being
correctly classified into the first two groups. The Southern region
oils are split into our two remaining groups, one containing all but
2 of the 25 North Apulian samples and 6 of the 36 Sicilian samples,
and the other group containing all the Southern oils. 
\begin{comment}
with North Apulia (23 out of 25
cases) and Sicilian oils

confusion matrix as in 
Table~\ref{tab:knob.sync.Olive-oil.kappa.1}.
\begin{table}[ht]
  \centering
  \caption{Confusion matrix for Olive-oil dataset, KNOB-SynC determine 4 cluster solution.} 
\label{tab:knob.sync.Olive-oil.kappa.1}
\begin{tabular}{llrrrr}
  \hline
Region & Area & 1 & 2 & 3 & 4 \\ 
\hline
Sardinia & Coast-Sardinia &  33 &   0 &   0 &   0 \\
& Inland-Sardinia &  65 &   0 &   0 &   0 \\ 
North&  East-Liguria &   0 &   0 &  50 &   0 \\ 
& West-Liguria &   0 &   0 &  50 &   0 \\
&  Umbria &   0 &   0 &  51 &   0 \\ 
South&  Calabria &   0 &  56 &   0 &   0 \\
& North-Apulia &   0 &   2 &   0 &  23 \\
&  South-Apulia &   0 & 206 &   0 &   0 \\
&  Sicily &   0 &  30 &   0 &   6 \\ 
  \hline
\end{tabular}
\end{table}
\end{comment}
In terms of clustering
performance, KNOB-SynC gets $\mR=0.55$ when compared to the true areal
grouping but $\mR=0.87$ when compared to the true regional grouping.
For this dataset DEMP ($\mR = 0.85;\hat C = 7$), DEMP+ ($\mR =
0.82;\hat C = 12$) and MMC ($\mR = 0.66;\hat C = 11$) are the top
three performers when comparing with the true areal grouping: all
other methods do worse than KNOB-SynC. However, in terms of
comparisons with the true regional grouping, KNOB-SynC is by far the best
performer. Overall, this clustering performance of KNOB-SynC
marginally trumps the 
performance of DEMP for the areal grouping and so can be considered to
be the most accurate in uncovering the group structure in the dataset. 
\begin{comment}

For this dataset, GSL-NN is the only method that identifies 9 groups $({\cal R} = 0.61)$ while FJ identifies 8 groups $({\cal R} = 0.54)$. CM $({\cal R} = 0.75)$, DEMP $({\cal R} = 0.82)$ and DEMP+ $({\cal R} = 0.85)$ are the best performers even though they identify only 7 groups. KNOB-SynC determines that there are 3 clusters. A closer look at the KNOB-SynC partitions reveals that oils from the southern areas of Calabria, Sicily and North and South Apulia are grouped together in our second cluster. Both Sardinian regions olive oils are identified very well by our methodology in a single group. Finally all the olive oils from the north are group together as well, i.e. East and West Liguria and Umbria.
\end{comment}

\subsubsection{Yeast Protein Localization}
The yeast protein localization dataset~\citep{nakai96} also obtained
from the UCIMLR was used by \citet{melnykov16} to illustrate the
application of DEMP+. This dataset is on the
localization of the proteins in yeast into one of 
($C=10$) sites and  has two attributes (presence of ``HDEL''
substring and peroxisomal targeting signal in the C-term) that are 
essentially binary and trinary, respectively. % however one of these
                                % combinations (0, 0.5) for 
                     % the two variables, has 1455 observations. We restrict attention to these 1455 observations and the 
Following \citet{melnykov16}, we drop these variables and use the other $p=6$ variables, namely signal sequence recognition score based on
(a) McGeoch's and (b) von Heijne's methods, (c) ALOM membrane spanning region
prediction score, and discriminant analysis scores of the amino acid
content of (d) N-terminal region (20 residues long) of mitochondrial and
non-mitochondrial proteins and (e)  vacuolar and extracellular
proteins and  (f) discriminant scores of nuclear localization signals
of nuclear and non-nuclear proteins. For this dataset, all methods perform poorly. KNOB-SynC ($\mR =
0.13;\hat C=6$) is the best performer, with the others being essentially
random allocations. Surprisingly, DEMP+ does very
poorly. (\citep{melnykov16} only used the first five variables in his
illustration and DEMP+'s clustering quality was not reported: we found no
appreciable performance even in that case). It
appears therefore  that groups may be difficult to find in the yeast
protein localization dataset  in a completely  unsupervised framework. 
\begin{comment}
This dataset is used to study the location of sites protein in yeast.
\begin{enumerate}
  \item Accession number for the SWISS-PROT database
  \item McGeoch's method for signal sequence recognition.
  \item von Heijne's method for signal sequence recognition.
  \item Score of the ALOM membrane spanning region prediction program.
  \item Score of discriminant analysis of the amino acid content of the N-terminal region (20 residues long) of mitochondrial and non-mitochondrial proteins.
  \item Presence of ``HDEL'' substring (thought to act as a signal for retention in the endoplasmic reticulum lumen). Binary attribute.
  \item Peroxisomal targeting signal in the C-terminus.
  \item Score of discriminant analysis of the amino acid content of vacuolar and extracellular proteins.
  \item Score of discriminant analysis of nuclear localization signals of nuclear and non-nuclear proteins.
\end{enumerate}

\begin{comment}

This data set contain 463 cytosolic or cytoskeletal, 429 nuclear, 244 mitochondrial, 163 membrane protein, no N-terminal signal, 51 membrame protein, uncleaved signal, 44 membrane protein, cleaved signal, 37 extracellular, 30 vacuolar, 20 peroxisomal, and 5 endoplasmic reticulum lumen. In this case, all the methods perform poorly with KNOB-SynC performing slightly best with a ${\cal R} = 0.13$. The minimum generalized overlap was obtained for $\kappa=3$, and a estimated $\hat{\genomega} = 0.017668 $. The final solution consist in 6 groups with one group containing mostly cytosolic or cytoskeletal, Membrane protein, no N-terminal signal, nuclear and most of vacuolar. The second group contain most of extracellular and other membrane proteins.

\begin{table}[h!]
  \centering
  \caption{Confusion matrix for yeast dataset, KNOB-SynC determine 6 cluster solution.}\label{tab:knob.sync.yeast-unscaled-6-kappa-3}
\begin{tabular}{lrrrrrr}
  \hline
  & 1 & 2 & 3 & 4 & 5 & 6 \\ 
  \hline
  Cytosolic or cytoskeletal & 415 &  33 &   4 &   8 &   0 &   3 \\ 
  Endoplasmic reticulum lumen &   0 &   0 &   5 &   0 &   0 &   0 \\ 
  Extracellular &   5 &   2 &  28 &   0 &   0 &   0 \\ 
  Membrane protein, cleaved signal &   1 &   0 &  41 &   0 &   2 &   0 \\ 
  Membrane protein, uncleaved signal &  20 &   2 &  29 &   0 &   0 &   0 \\ 
  Membrane protein, no N-terminal signal & 152 &   6 &   3 &   2 &   0 &   0 \\ 
  Mitochondrial &  99 & 132 &  13 &   0 &   0 &   0 \\ 
  Nuclear & 359 &  32 &   4 &  34 &   0 &   0 \\ 
  Peroxisomal &  16 &   2 &   2 &   0 &   0 &   0 \\ 
  Vacuolar &  23 &   2 &   5 &   0 &   0 &   0 \\ 
   \hline
\end{tabular}
\end{table}
\end{comment}


\subsubsection{Image Segmentation}
 \label{sec:app.image}
 The image segmentation dataset, also available from the UCIMLR, is on 19 
 attributes of the scene in each $3\times 3$ 
 image, as per hand-drawn classification  into BRICKFACE,
 CEMENT, FOLIAGE, GRASS, PATH, SKY and WINDOW. (Thus $C=7$.) We
 combine the training 
 and test datasets to obtain 330 instances of each scene, so
 $n=2310$. %Nine of the attributes can be linearly explained by the
 % others, so we discaed  these attributes. Further,     %eight principal
 There is a lot of redundancy in the attributes so we reduce the
 dataset to eight principal components (PCs) that explains at least 99.9\%
 of the total variability in the dataset. We use PCs computed on the
correlation matrix because of the wide range in scales for the 19
attributes. The KNOB-SynC solution found $\hat C = 12$ clusters, with
 $\mR=0.55$. The confusion matrix
 (Table~\ref{tab:knob.sync.Image-scaledpc-8-kappa-3}) indicates that
 the SKY scene is perfectly identified while GRASS and, to a lesser
 extent,  PATH and CEMENT, are fairly  well-identified. 
\begin{table}[h!]
  \centering
  \caption{Confusion matrix of the KNOB-SynC grouping against the true for
    the Image dataset.}
\label{tab:knob.sync.Image-scaledpc-8-kappa-3}
  \begin{tabular}{lrrrrrrrrrrrr}
    \hline
    & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\ 
    \hline
    BRICKFACE & 330 & 0 & 0 &  0 & 0 & 0 & 0 &   0 &   0 &   0 &   0 &   0 \\ 
    CEMENT &  42 &  257 & 0 & 4  &   0 &   27 &  0 &   0 &   0 &   0 &   0 &   0 \\ 
    FOLIAGE & 300 &  5 & 0 & 0 & 0 & 5 &  2  &   7 &   3 &   1 &   3 &   4 \\ 
    GRASS &   1 &  0 &   327 &   0 & 0 & 2 & 0 &   0 &   0 &   0 &   0 &   0 \\ 
    PATH &   0 & 0 &   0 &   269 &   0 &  61 & 0& 0 &   0 &   0 &   0 &   0 \\ 
    SKY &   0 &   0 & 0 &   0 &   330 &   0 &   0 &   0 &   0 &   0 &   0 &   0 \\ 
    WINDOW & 309 &  13 &   0 &  0 &   0 &   8 & 0& 0 &   0 &   0 &   0 &   0 \\ 
   \hline
  \end{tabular}
\end{table}
\begin{comment}
\begin{table}[ht]
\caption{Confusion matrix for EAC with ${\cal R}=0.59$.}
{\tiny
\begin{tabular}{rrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
  \hline
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 &
17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & 28 & 29 & 30 & 31 &
32 & 33 & 34 & 35 & 36 & 37 & 38 & 39 & 40 \\
  \hline
BRICKFACE &  66 &  31 &  41 &  37 & 146 &   8 &   0 &   0 &   0 &   0 &   0
&   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &
0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   1 &   0 &   0
&   0 &   0 &   0 &   0 \\
  CEMENT &   0 &   0 &   0 &   0 &  32 &  12 &   0 &   0 &   0 &   0 &   0
&   6 &   0 &   2 &   0 & 215 &  18 &  14 &  13 &   7 &   0 &   0 &   5 &
0 &   0 &   0 &   1 &   0 &   0 &   1 &   0 &   1 &   3 &   0 &   0 &   0
&   0 &   0 &   0 &   0 \\
  FOLIAGE &   0 &   0 &   5 &   0 &  52 & 220 &   0 &   0 &   0 &   0 &   3
&   3 &   6 &  13 &   4 &   0 &   2 &   0 &   0 &   0 &   1 &   0 &   0 &
0 &   0 &   0 &   0 &   5 &   1 &   0 &   0 &   3 &   1 &   0 &   3 &   3
&   3 &   1 &   1 &   0 \\
  GRASS &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0
&   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   3 &
0 & 327 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0
&   0 &   0 &   0 &   0 \\
  PATH &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0
&   7 &   0 &   0 &   0 &   0 &  28 &   0 &   0 &   0 &   0 &   0 & 292 &
3 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0
&   0 &   0 &   0 &   0 \\
  SKY &   0 &   0 &   0 &   0 &   0 &   0 & 289 &  28 &   9 &   3 &   0 &
0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0
&   0 &   0 &   0 &   0 &   0 &   0 &   1 &   0 &   0 &   0 &   0 &   0 &
0 &   0 &   0 &   0 \\
  WINDOW &   1 &   0 &   1 &   0 &  62 & 187 &   0 &   0 &   0 &   0 &   0
&   0 &   0 &  18 &   0 &  10 &   6 &   4 &   0 &   1 &  19 &  17 &   0 &
0 &   0 &   3 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0
&   0 &   0 &   0 &   1 \\
   \hline

\end{tabular}
}
\end{table}
\end{comment}
EAC does slightly better than KNOB-Sync ($\mR = 0.59$) but identifies 40
groups. Inspection of that grouping indicates many small groups but
also  difficulty in separating FOLIAGE and WINDOW, placing them
together in one group. Further, BRICKFACE is split 
into five groups, four of which are predominantly of this kind, but
the fifth group is unable to distinguish 146 observations of BRICKFACE
from 32, 52 and 62 observations of CEMENT, FOLIAGE and WINDOW,
respectively. 

\subsubsection{Acute Lymphoblastic Leukemia}\label{sec:sim.ALL}
The Acute Lymphoblastic Leukemia (ALL) training dataset of \citet{yeohetal02}
was used by \citet{stuetzleandnugent10} to illustrate GSL-NN in a
high-dimensional small sample size framework. We used the
standardized dataset in 
\citet{stuetzleandnugent10} that measured the oligonucleotide 
expression levels of the 1000 highest-varying genes in 215 patients
suffering from one of seven leukemia subtypes, namely, T-ALL,
E2A-PBX1, BCR-ABL, TEL-AML1, MLL rearrangement, Hyperploid $> 50$
chromosomes, or an unknown category labeled OTHER. Some subtypes have
very few cases: for instance, only 9, 14 and 18 patients are of type
BCR-ABL, MLL and E2A-PBX1, respectively. For this
dataset, we used $m=42$ KPCs for all methods but for GSL-NN. KNOB-SynC
identifies $\hat C=16$ groups, with
$\mR=0.59$. Table~\ref{tab:knob.sync.ALL-Nugent-kPCA-42}  
\begin{table}[h]
  \centering
  \caption{Confusion matrix of the KNOB-SynC grouping against
    the true for the ALL dataset.}\label{tab:knob.sync.ALL-Nugent-kPCA-42}
\begin{tabular}{lrrrrrrrrrrrrrrrr}
  \hline
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 \\ 
  \hline
  Hyperdiploid $\!>\!$ 50\! &35&0&0&0&2 & 0 &   0 &   2 &   1 &   1 &  0 &   0 &   0 &   1 &   0 &   0 \\ 
  E2A-PBX1 &           0 &17&0&0&0&0 & 0 & 0 & 0 &   0 &   1 &   1 &   0 &   0 &   0 &   0 \\ 
  OTHERS &   0 &   0 &  51 &   0 &   0 &   0 &   0 &   0 &   0 &  1 &   1 &   0 &   0 &   0 &   0 &   0 \\ 
  BCR-ABL &   2 &   0 &   0 &   3 &   4 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 \\ 
  TEL-AML1 &   7 &   2 &   6 &   0 &  12 &   8 &   0 &   1 &   5 &   0 &   0 &   1 &   9 &   1 &   0 &   0 \\ 
  MLL &   0 &   4 &   0 &   0 &   0 &   10 &   0 &   0 &   0 &   0 &  0 &   0 &   0 &   0 &   0 &   0 \\ 
  T-ALL &   0 &   0 &   0 &   0 &   0 &   0 &  24 &   0 &   0 &   0 &   0 &   0 &   0 & 0 &   3 &   1 \\ 
   \hline
\end{tabular}
\end{table}
presents the confusion matrix containing the number of cases a patient of a 
leukemia subtype was assigned to a KNOB-SynC group. Three of the
syncytial clustered groups have only one observation, another two have
two observations and three other groups have three observations. The
TEL-AML1 and BCR-ABL leukemia subtypes are scattered over multiple
groups, but the other subtypes are fairly  well-identified and largely
get assigned to their own KNOB-SynC groups. The alternative methods
perform mildly to substantially worse. GSL-NN, spectral clustering,
EAC and kernel $k$-means ($C=7$, given) have similar performance while
K-mH, DEMP and DEMP+ do poorly in accurately finding structure in the
dataset. 
\begin{comment}
\begin{table}[h]
  \centering
  \caption{Confusion matrix for E.coli dataset, KNOB-SynC determine 12 cluster solution.}  \label{tab:knob.sync.Ecoli-kPCA-10}
\begin{tabular}{lrrrrrrrrrrrr}
  \hline
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\ 
  \hline
  cytoplasm % Cytoplasm
  & 132 &   3 &   0 &   0 &   0 &   3 &   4 &   0 &   0 &   0 &   0 &   1 \\ 
  inner membrane, no signal sequence %Inner membrane without signal sequence
  &   2 &  51 &   0 &  12 &   0 &   0 &   0 &   3 &   4 &   3 &   1 &   0 \\ 
 % Inner membrane lipoprotein &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 \\ 
  imS %Inner membrane, cleavable signal sequence
  &   0 &   1 &   1 &   0 &   0 &  0 &   0 &   0 &   0 &   0 &   0 &   0 \\ 
  imU %Inner membrane, uncleavable signal sequence
  &   0 &  10 &   0 &  23 &   0 &   0 &   0 &   0 &   0 &   0 &   1 &   0 \\ 
  om %Outer membrane
  &   0 &   0 &   0 &   0 &  16 &   2 &   0 &   0 &   0 &   0 &   0 &   1 \\ 
%  Outer membrane lipoprotein &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 \\ 
  pp %Perisplasm
  &   3 &   1 &  0 &   0 &   2 &   38 &   0 &   0 &   0 &   0 &   0 &   8 \\ 
   \hline
\end{tabular}
\end{table}
\end{comment}
\subsubsection{Zipcode images}
The zipcode images~\citep{stuetzleandnugent10} dataset consists of $n=2000$
$16\times 16$ images of handwritten Hindu-Arabic numerals and is our
second higher-dimensional example. As in the ALL dataset of
Section~\ref{sec:sim.ALL}, we normalized the observations to have zero mean and
variance so that the Euclidean distance between any two normalized
images is negatively and linearly related to the correlation between
their pixels. We extracted and used the first $m=33$ KPCs for all
algorithms but GSL-NN. KNOB-SynC identified 9 groups and had the best
clustering performance ($\mR=0.76$). 
\begin{figure}[h] 
  \centering
  \includegraphics[width = \textwidth]{figures/zipdigits-tall-crop}
  \caption{KNOB-SynC groups, with colormap indicating group, of the Zipcode dataset.}
  \label{fig:zip}
\end{figure}
Figure~\ref{fig:zip} displays the 2000 digits with color scale
for each of the  9 KNOB-SynC groups. While outliers abound in almost
all groups, there is good agreement with 0, 1, 2, the
leaner 8s and, less-so, 3 and 6 largely correctly identified. The digit 2
is placed in two groups, of the leaner and the rounded versions,
respectively. The group where 3 predominates also has some 5's and 8's 
but the categorization makes visual sense. Another group is composed
largely of 4s, 7s and 9s but the placement also appears visually
explainable. Clearer and straighter  7s and 9s are placed
in a separate group. Our partitioning finds it harder to distinguish
between 5 and 6 but here also the commonality of the strokes in the
digits assigned to this group explains this categorization. 
The alternative methods all perform moderately ($\mR=0.55. \hat
C=22$ for K-mH; $\mR=0.54$, $\hat C=5$ and $7$, respectively for both
spectral clustering and GSL-NN) to substantially worse. Thus
KNOB-SynC  is the best performer for this dataset and also provides
interpretable results. We comment that the application of all methods
to this dataset has been entirely unsupervised: methodologies that
also account for spatial context and pixel neighborhood have the
potential to further improve  classification but are outside the
purview of this paper.  
\subsubsection{Handwritten Pen-digits}\label{sec:experiment.pendigits}
The Handwritten Pen-digits
dataset~\citep{alimoglu96,alimogluandalpaydin96} available at  the 
\begin{table}[ht]
\vspace{-0.2in}
  \centering
  \caption{Confusion matrix for the Handwritten Pen-digits dataset.} 
\label{tab:knob.sync.pendigits}
\begin{tabular}{rrrrrrrrrrrrrr}
  \hline
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 &13\\ 
  \hline
  0 & 1119 &  1  &   2 &   0 &  17 &   0 &   2 &   0 & 0 & 0 & 1  & 0 & 1 \\ 
  1 &   0 & 640 &  359 &  138 &  2 &   0 &   0 &  3 & 1 & 0 & 0 & 0 & 0\\
  2 &   0 & 2 & 1140 &   1 & 0 & 0 & 0 & 0 &  1 & 0 & 0 & 0 & 0\\
  3 &   0 & 14 &  2 & 1036 &1    & 0 & 2 &  0 & 0 & 0 & 0 & 0 & 0 \\
  4 &  0 &   12 &   1 &  3 & 1113 &  0 & 14 & 1 & 0  & 0 & 0 & 0 & 0\\
  5 &   0 &   0 &   0 & 246 &  1 & 624 & 181 & 0 & 0 & 2& 1& 0 &0\\
  6 &   0 & 0 & 2 & 1 & 2 & 1 & 0 & 1050 & 0 & 0 & 0 &0   0 &   0 \\
  7 &  0 &  144 &   8 &   0 & 0 &   0 & 0 & 0 & 911 & 0 & 0 & 79 &0\\
  8 &  2 &  0 & 70 & 33 & 0 & 2 & 0 & 0 &  4 & 372 & 524 & 48 & 0\\
  9 &  0 &  9 &  0 & 311 & 13 & 0 & 697 & 0 &   0 & 0 & 1 & 0 & 24 \\
   \hline
\end{tabular}
\end{table}
UCIMLR is a larger dataset that measured 16 attributes from 250 
handwritten samples of 30 writers. (There are $n=10,992$ records
because eight samples are unavailable.) Following \citet{petersonetal17}, 
we used the first 7 principal component scores that explained 90\% of 
the total variation in the dataset. Because of the size of the dataset, our
comparisons are only with EAC and K-mH (the other methods either took
a very long time or threw up errors).  KNOB-SynC found 13 groups and
was the best performer ($\mR=0.69$). It found 0, 2, 3, 4, 6 and  7
fairly well but identifying 1, 5 and 9 
was more difficult~(Table \ref{tab:knob.sync.pendigits}). It also
suggested that  multiple types of 8. EAC identified the correct number
of groups but performed
very poorly $({\cal R} = 0.1)$ while K-mH identified $\hat C = 24$ with
$({\cal R} = 0.64)$. 
\begin{comment}
\begin{table}[ht]
\centering
\caption{Confusion matrix for eight clusters of Image Segmentation using KNOB-SynC. Rows represent the origin and columns each represent one of the eigth identified clusters.} 
\label{tab:conf.mat.image.train}
\begin{tabular}{lcccccccc}
  \hline
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\ 
  \hline
  BRICKFACE &  29 &   1 &   0 &   0 &   0 &   0 &   0 &   0 \\ 
  CEMENT &  27 &   1 &   0 &   0 &   1 &   0 &   1 &   0 \\ 
  FOLIAGE &  24 &   1 &   0 &   1 &   1 &   2 &   1 &   0 \\ 
  GRASS &  23 &   0 &   0 &   0 &   0 &   0 &   0 &   7 \\ 
  PATH &  23 &   2 &   0 &   0 &   5 &   0 &   0 &   0 \\ 
  SKY &   0 &   0 &  30 &   0 &   0 &   0 &   0 &   0 \\ 
  WINDOW &  30 &   0 &   0 &   0 &   0 &   0 &   0 &   0 \\ 
   \hline
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Confusion matrix for fourth clusters of Image Segmentation test using KNOB-SynC. Rows represent the origin and columns each represent one of the fourth identified clusters.} 
\label{tab:conf.mat.image.test}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrr}
  \hline
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 \\ 
  \hline
BRICKFACE &   0 &   0 &   0 & 246 &  43 &   0 &   0 &   3 &   8 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 \\ 
  CEMENT &   0 &   0 &   0 & 238 &  38 &   5 &   1 &   1 &   5 &   0 &   0 &   2 &   7 &   3 & 2  0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 \\ 
  FOLIAGE &   0 &   0 &   0 & 233 &  26 &   1 &   1 &  17 &   0 &   4 &   0 &   0 &   0 &   1 &   2 &   1 &   3 &   3 &   2 &   2 &   3 &   1 \\ 
  GRASS & 231 &  63 &   3 &   1 &   1 &   0 &   1 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 \\ 
  PATH &   0 &   0 &   0 & 246 &  31 &  20 &   3 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 \\ 
  SKY &   0 &   0 &   0 &   0 &   0 &   1 &   0 &   0 &   0 &   0 & 275 &  24 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 \\ 
  WINDOW &   0 &   0 &   0 & 276 &  12 &   1 &   0 &   8 &   1 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   0 &   2 &   0 &   0 &   0 &   0 \\ 
   \hline
\end{tabular}
\end{table}
\end{comment}
\subsubsection{Summary of Performance}\label{sec:HD}
 Figure~\ref{fig:AR.HD} and Table~\ref{tab:AR.HD} summarize performance of 
all methods on the higher-dimensional examples. It is easy
to see that KNOB-SynC is almost always among the top
\begin{figure}[h!]
  \centering
  \includegraphics[width = \textwidth]{figures/AR-High-Dimensional-v3-crop}
  \caption{Clustering performance, in terms of the Adjusted Rand
    Index, of KNOB-SynC and its competitors on all high-dimensional datasets.}
  \label{fig:AR.HD}
\end{figure}
performers. Indeed, KNOB-SynC had the lowest average difference in
$\mR$ from that of the best performing method  over all datasets
(Table~\ref{tab:AR.HD}).
The other methods perform similarly on
the average, with EAC being the better of them, on the average. 
\begin{table*}[h!]
  \centering
  \caption{Performance, in terms of $\mR$ and $\hat C$ of all methods
    in the higher-dimensional datasets. Notations are as in
    Table~\ref{tab:AR.HD}.} 
  \label{tab:AR.HD}
  \begin{tabular}{lcccccccccc}
    \hline\hline
    % \multicolumn{11}{c}{Adjusted Rand Index ${\cal R}$ and estimated number of groups $\hat{K}$} \\
    % \cline{3-11}
    Dataset  & & KNS & K-mH& DM & DM+ & MMC & EAC & GSN  & SpC &
                                                                 k-$k$m \\
    $(n,p,K)$ & &  & &  & &  &  &  & &  \\ 
    \hline\hline
    Simplex-7 &${\cal R}$ & 0.97 & 0.97 & 0.97 & 0.97 & 0.97 & 0.94 & 0.94 & 0.92 & 0.94\\
    ($560,7,7$) &$\hat{C}$ & 7 & 7 & 7 & 7 & 7 & 6 & 7 & 7 & \\
    \hline
    E.coli &${\cal R}$ & 0.72 &  0.63 & 0.70 & 0.68 & 0.59 & 0.77 & 0.03 & 0.26 & 0.45 \\ 
    ($336,7,7 $)&$\hat{C}$ & 9 &     4 & 4 & 4 & 8 & 10 & 16 & 15 &  \\ 
    \hline
    Wines &${\cal R}$ & 0.55 & 0.62 & 0.52 & 0.5 & 0.67 & 0.60 & 0.38 & 0.43 &0.6 \\
    ($178,13, 3$) &$\hat{C}$ & 24 & 6 & 7 & 7 & 5 & 9 & 15 & 7 & \\
    \hline
    Olive-Area&${\cal R}$ & 0.55 & 0.56 & 0.85 & 0.82 & 0.66 & 0.55 & 0.51 & 0.48 & 0.56\\
    ($572,8,9$) &$\hat{C}$ & 4 & 8 & 7 & 12 & 11 & 14 & 5 & 18 & \\
    \hline
    %%km-H should be 
    Olive-Region &${\cal R}$ & 0.87 & 0.4 & 0.44 & 0.46 & 0.39 & 0.46 & 0.48 & 0.23 & 0.39\\
    ($572,8,3$) &$\hat{C}$ & 4 & 8  & 7 & 12 & 11 & 14 & 16 & 18 & \\
    \hline
     Yeast &${\cal R}$ & 0.13& 0.05 & -0.008 & -0.01 & 0.04 & 0.01 & 0.0031 & 0.05 & 0.09\\
    ($1484,8,10$) &$\hat{C}$  & 6 & 7 & 5 & 5 & 33 & 38 & 33 & 39 &  \\ 
    \hline
   Image &${\cal R}$ & 0.54 & 0.48 & 0.49 & 0.46 & 0.28 & 0.59 & 0.10 & 0.22 & 0.52  \\
    ($2310,19, 7$)  &$\hat{C}$ &  12 &  17  & 18 & 17 & 46 & 40 & 48 & 45 & \\
    \hline
    ALL &${\cal R}$   & 0.59 & 0.19 & 0.14 & 0.14 & 0.35 & 0.53 & 0.54 & 0.55 & 0.5 \\ 
    ($215,1000, 7$) &$\hat{C}$ & 16 & 18 & 6 & 6 & 9 & 9 & 5 & 12 &  \\ 
    \hline
   % ALL (complete) &${\cal R}$ & 0.25 & 0.15 & 0.14 & 0.14 & 0.52 & 0.52 & 0.13 & 0.64 & 0.5\\
  %  ($327,12558, 7$) &$\hat{C}$ & 5 & 6 & 6 & 6 & 13 & 9 & 13 & 12 & 7\\
  %  \hline
  %  Glass &${\cal R}$ & 0.27 & 0.43 & 0.42 & 0.12 & 0.1 & 0.1 & 0.16 & 0.37 & 0.16\\
  %  ($214,9, 7$)  &$\hat{C}$ & 10 & 11 & 10 & 41 & 4 & 4 & 15 & 3 & 5\\
  %  \hline
    % Iris&${\cal R}$ & 1.00 & 1.00 & 1.00 & 0.77 & 1.00 & 0.67 & 1.00 & 1.00 & 0.98\\
    % &$\hat{K}$ & 2 & 2 & 3 & 2 & 4 & 2 & 3 & 2 & 3\\
    % \hline
    Zipcode&${\cal R}$ & 0.76 & 0.55 & 0.35 & 0.33 & 0.01 & 0.21 & 0.54 & 0.54 & 0.00\\
    ($2000,256,10$)&$\hat{C}$ & 9 & 22 & 36 & 33 & 1 & 45 & 7 & 5 & \\
    \hline
    Pendigits &${\cal R}$ & 0.69 & 0.64 & - & - & - & 0.10 & - & 0.59 & 0.47 \\
    ($10992,16,10$)  &$\hat{C}$ & 13 & 24 & - & - & - & 10 & - & 17 & \\
    \hline \hline
    $\bar{\cal D}$ & & 0.05 & 0.23 & 0.20 & 0.21 & 0.28 & 0.18 & 0.24 & 0.26 & 0.24 \\ 
    ${\cal D}_\sigma$ &  & 0.1 & 0.20 & 0.18 & 0.17 & 0.25 & 0.18 & 0.18 & 0.20 & 0.25 \\ 
%Median ${\cal D}$&  & 0.00 & 0.21 & 0.15 & 0.15 & 0.24 & 0.12 & 0.22 & 0.24 & 0.09 \\  
%IQR ${\cal D}$ & & 0.05 & 0.23 & 0.31 & 0.28 & 0.39 & 0.24 & 0.21 & 0.29 & 0.27 \\
    \hline\hline
  \end{tabular}
\end{table*}

The results of our experiments on multiple kinds of datasets in two
and higher dimensions indicate good performance for the KNOB-SynC
algorithm. We now apply the methodology to two real-world
applications. 
